Do LLMs Recognize Your Preferences? Evaluating Personalized Preference Following in LLMs

Large Language Models (LLMs) are increasingly used as chatbots, yet their ability to personalize responses to user preferences remains limited. We introduce PrefEval, a benchmark for evaluating LLMs' ability to infer, memorize and adhere to user preferences in a long-context conversational setting. PrefEval comprises 3,000 manually curated user preference and query pairs spanning 20 topics. PrefEval contains user personalization or preference information in both explicit and implicit forms, and evaluates LLM performance using a generation and a classification task. With PrefEval, we evaluated the aforementioned preference following capabilities of 10 open-source and proprietary LLMs in multi-session conversations with varying context lengths up to 100k tokens. We benchmark with various prompting, iterative feedback, and retrieval-augmented generation methods. Our benchmarking effort reveals that state-of-the-art LLMs face significant challenges in proactively following users' preferences during conversations. In particular, in zero-shot settings, preference following accuracy falls below 10% at merely 10 turns (~3k tokens) across most evaluated models. Even with advanced prompting and retrieval methods, preference following still deteriorates in long-context conversations. Furthermore, we show that fine-tuning on PrefEval significantly improves performance. We believe PrefEval serves as a valuable resource for measuring, understanding, and enhancing LLMs' preference following abilities, paving the way for personalized conversational agents. Our code and dataset are available at https://prefeval.github.io/.

==> sections/related_works_draft.tex <==
Personalization for dialogue systems aims to endow a text
generation system with particular personality
traits.

\citet{zhang-etal-2018-personalizing} condition on user profile information to provide more personalized chit-chat responses. Focuse on more engaging chit-chat dialogue agents by endowing
them with a configurable, but persistent persona. profile can be stored in a memory-augmented neural network. present the PERSONA-CHAT dataset, a new dialogue dataset consisting of 162,064 utterances between crowdworkers who were randomly paired
and each asked to act the part of a given provided
persona (randomly assigned, and created by another set of crowdworkers). conditioning the agent with
persona information gives improved prediction of
the next dialogue utterance. Metric: next utterance prediction conditioned on the persona based dialogue. 

\citet{mazare-etal-2018-training} following the above work, introduce a new dataset providing 5 million personas and 700 million persona-based dialogues to train on. 

instead of using synthetic or labelled personzlaied dialogue, \citet{wu-etal-2021-personalized} collected personalized responses for questions on Reddit by utilizing personalized user profiles and posting histories in a single-turn dialog setting. 

\citet{ao-etal-2021-pens} focuses on personalized news headline generation problem whose goal is to output a user-specific title.


\citet{zhong-etal-2022-less} learn to extract the most informative segments from the user's history for personalization.

Other types of personalization generation tasks:
\citet{salemi2023lamp} personalizing text classification/generation such as citation identification, tweet paragraphing.


personalize large language models themselves to embody a particular persona, where the goal is to generate output that mimics the speaking style and patterns associated with the provided persona metadata \citep{vincent2023reference}.

